SMPLer-X: Scaling Up Expressive Human Pose and Shape Estimation

Expressive human pose and shape estimation (EHPS) unifies body, hands, and face motion capture with numerous applications. Despite encouraging progress, current state-of-the-art methods still depend largely on a confined set of training datasets. In this work, we investigate scaling up EHPS towards the first generalist foundation model (dubbed SMPLer-X), with up to ViT-Huge as the backbone and training with up to 4.5M instances from diverse data sources. With big data and the large model, SMPLer-X exhibits strong performance across diverse test benchmarks and excellent transferability to even unseen environments. 1) For the data scaling, we perform a systematic investigation on 32 EHPS datasets, including a wide range of scenarios that a model trained on any single dataset cannot handle. More importantly, capitalizing on insights obtained from the extensive benchmarking process, we optimize our training scheme and select datasets that lead to a significant leap in EHPS capabilities. 2) For the model scaling, we take advantage of vision transformers to study the scaling law of model sizes in EHPS. Moreover, our finetuning strategy turn SMPLer-X into specialist models, allowing them to achieve further performance boosts. Notably, our foundation model SMPLer-X consistently delivers state-of-the-art results on seven benchmarks such as AGORA (107.2 mm NMVE), UBody (57.4 mm PVE), EgoBody (63.6 mm PVE), and EHF (62.3 mm PVE without finetuning). Homepage: https://caizhongang.github.io/projects/SMPLer-X/

==> figures/ranking_correlation.tex <==
% \begin{wrapfigure}{r}{0.4\textwidth}
\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\linewidth]{images/ranking_correlation.pdf}
  \vspace{-0.3cm}
  \caption{\textbf{Correlation of benchmark datasets}. For each dataset, we train a model on its training set and evaluate its performance on the \textit{training} sets of seven benchmark datasets: 3DPW, AGORA, EgoBody (EgoSet), UBody, and ARCTIC and DNA-Rendering (High-resolution set). Datasets are then ranked by MPE. We study the correlation of benchmark datasets by their rankings among all datasets.}
  \label{fig:ranking_correlation}
\end{figure}
% \end{wrapfigure}


==> tables/full_results.tex <==


\begin{sidewaystable}
    \centering
    \caption{Complete results of individual dataset benchmark with the same setting as Table 1 in the main paper. We train a model for each dataset on its training set and evaluate its performance on the \textit{training} sets of six benchmarks. Top-1 values are bolded, and the rest of the Top-5 are underlined. Unit: mm.}
    \label{tab:full_res}
    \resizebox{1.05\textwidth}{!}{
    \begin{tabular}{l|cccccc|cccccccc|cccccccc|cc|cccccccc|cccccccc}
    
    \toprule 
    & \multicolumn{6}{c}{AGORA~\cite{patel2021agora}} & \multicolumn{8}{c}{UBody~\cite{lin2023one}} & 
    \multicolumn{8}{c}{EgoBody~\cite{zhang2022egobody}} & \multicolumn{2}{c}{3DPW~\cite{von2018recovering}} & \multicolumn{8}{c}{ARCTIC~\cite{fan2023arctic}} & \multicolumn{8}{c}{DNA-Rendering~\cite{renbody} } \\
    \cmidrule(lr){2-7} \cmidrule(lr){8-15} \cmidrule(lr){16-23} \cmidrule(lr){24-25} \cmidrule(lr){26-33} \cmidrule(lr){34-41}
    
    & \multicolumn{3}{c}{PA-PVE$\downarrow$} & \multicolumn{3}{c}{PVE$\downarrow$} & 
    \multicolumn{3}{c}{PA-PVE$\downarrow$} & \multicolumn{3}{c}{PVE$\downarrow$} & \multicolumn{2}{c}{PA-MPJPE$\downarrow$} &
    \multicolumn{3}{c}{PA-PVE$\downarrow$} & \multicolumn{3}{c}{PVE$\downarrow$} & \multicolumn{2}{c}{PA-MPJPE$\downarrow$} &
    \multicolumn{2}{c}{PA-MPJPE$\downarrow$} &
    \multicolumn{3}{c}{PA-PVE$\downarrow$} & \multicolumn{3}{c}{PVE$\downarrow$} & \multicolumn{2}{c}{PA-MPJPE$\downarrow$} &
    \multicolumn{3}{c}{PA-PVE$\downarrow$} & \multicolumn{3}{c}{PVE$\downarrow$} & \multicolumn{2}{c}{PA-MPJPE$\downarrow$} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
    \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-15} 
    \cmidrule(lr){16-18} \cmidrule(lr){19-21} \cmidrule(lr){22-23}
    \cmidrule(lr){24-25} 
    \cmidrule(lr){26-28} \cmidrule(lr){29-31} \cmidrule(lr){32-33}
    \cmidrule(lr){34-36} \cmidrule(lr){37-39} \cmidrule(lr){40-41}   
        
      Dataset &  All &  Hand &  Face &  All &  Hand &  Face &  All &  Hand &  Face &  All &  Hand &  Face &  Body &  Hand &  All &  Hand &  Face &  All &  Hand &  Face &  Body &  Hand &  Body &  Body &  All &  Hand &  Face &  All &  Hand &  Face &  Body &  Hand &  All &  Hand &  Face &  All &  Hand &  Face &  Body &  Hand \\

      \midrule
        MSCOCO~\cite{lin2014microsoft} & 75.7 & \underline{12.0} & \underline{5.1} & 174.4 & 76.5 & 79.1 & \underline{42.2} & \underline{10.3} & \underline{2.9} & \underline{94.5} & \underline{47.3} & \underline{28.2} & \underline{49.3} & \underline{10.6} & \underline{53.4} & 10.4 & \underline{3.7} & \underline{114.4} & \underline{49.8} & \underline{42.7} & \underline{62.3} & 10.7 & 102.7 & 69.3 & \underline{62.3} & 17.2 & 4.9 & \underline{122.7} & \underline{54.4} & 56.8 & \underline{69.0} & 17.0 & 59.5 & \underline{9.4} & \underline{3.7} & 104.3 & 52.5 & 49.7 & 60.8 & \underline{9.5} \\
        
        BEDLAM~\cite{black2023bedlam} & \underline{74.8} & \underline{12.1} & \underline{5.6} & \underline{159.0} & \underline{72.2} & \underline{67.8} & 64.9 & \underline{10.8} & 5.0 & 133.6 & \underline{60.8} & \underline{39.4}& 85.3 & \underline{11.0} & 59.6 & \underline{9.7} & 4.8 & 110.3 & \underline{47.7} & \underline{42.4} & \underline{79.0} & \underline{9.9} & {103.0} & 78.1 & \underline{65.4} & 18.5 & \underline{3.5} & \underline{103.6} & 58.5 & \underline{39.9} & 77.7 & 18.3 & 57.9 & 10.2 & 4.4 & \underline{91.0} & \underline{49.2} & \underline{42.4} & 68.8 & 10.2 \\
        
        GTA-Human~\cite{cai2021playing} & \underline{69.1} & 15.6 & 6.1 & \underline{153.4} & \underline{71.4} & \underline{69.5} & 66.3 & 18.9 & 4.9 & 136.5 & 67.1 & 52.0 & 84.9 & 19.1 & \underline{57.3} & 17.6 & 4.6 & 124.4 & 52.6 & 54.0 & \underline{66.5} & 18.1 & \textbf{93.5} & \textbf{59.4} & \underline{61.0} & \underline{15.6} & 5.6 & 132.8 & \underline{50.8} & 70.7 & \underline{66.7} & \underline{15.6} & \underline{52.6} & 12.8 & 4.5 & 107.6 & \underline{48.6} & 52.5 & \underline{57.1} & 13.0 \\
        
        SPEC~\cite{kocabas2021spec} & \underline{73.7} & 20.2 & 30.1 & \underline{137.7} & \underline{64.9} & 78.0 & 68.3 & 21.0 & 28.8 & 129.6 & \underline{59.9} & 59.5 & 78.5 & 19.4 & 65.6 & 19.6 & 28.8 & 126.7 & \underline{49.1} & 62.2 & 69.2 & 18.0 & 114.2 & 68.0 & 70.4 & 23.5 & 30.1 & 137.5 & \underline{54.1} & 56.3 & \underline{70.6} & 22.6 & 65.2 & 17.9 & 29.9 & 112.5 & \underline{48.7} & 55.2 & 64.1 & 16.1 \\
        
        AGORA~\cite{patel2021agora} & \textbf{40.3} & \textbf{7.6} & \textbf{4.0} & \textbf{83.4} & \textbf{42.1} & \textbf{38.5} & 68.1 & 11.4 & 4.6 & 135.1 & 64.9 & 51.7 & 91.5 & 11.6 & 66.4 & 10.9 & \underline{4.1} & 149.0 & 61.2 & 61.1 & 78.9 & 11.2 & 111.4 & 65.6 & \underline{69.2} & \underline{16.6} & \textbf{3.1} & 143.1 & 57.3 & 57.7 & 77.5 & 16.5 & \underline{51.4} & 10.6 & \underline{3.9} & 126.8 & 53.1 & 50.8 & \underline{52.8} & 10.7 \\
        
        SynBody~\cite{yang2023synbody} & \underline{74.1} & 20.0 & \underline{5.6} & \underline{155.2} & \underline{72.6} & \underline{69.4} & 75.5 & 21.1 & 5.2 & 141.6 & 73.2 & 49.9 & 87.1 & 22.1 & 79.1 & 23.2 & 4.9 & 137.0 & 65.9 & 59.5 & 91.2 & 24.5 & 99.4 & 69.6 & 80.7 & \underline{15.7} & \textbf{3.1} & 155.6 & 59.0 & 72.0 & 87.8 & \underline{16.0} & \underline{55.1} & 18.2 & 4.5 & \underline{91.5} & 51.3 & 46.2 & 60.2 & 19.0 \\
        
        PoseTrack~\cite{andriluka2018posetrack} & 86.7 & 21.0 & 16.3 & 177.9 & 89.0 & 88.8 & \underline{56.8} & 21.0 & 16.7 & \underline{119.2} & 66.6 & 55.7 & \underline{62.2} & 19.6 & 64.4 & 18.6 & 15.4 & 122.9 & 63.0 & 61.5 & 68.8 & 17.2 & 115.9 & 81.5 & 71.1 & 24.8 & 16.8 & 127.7 & 66.7 & 57.0 & 81.3 & 23.8 & 74.5 & 20.9 & 15.7 & 123.5 & 73.0 & 59.4 & 76.8 & 19.4 \\
        
        Egobody-EgoSet~\cite{zhang2022egobody} & 92.6 & 12.6 & \underline{5.6} & 188.0 & 93.9 & 86.3 & \underline{61.7} & 11.6 & \underline{4.1}& \underline{117.0} & \underline{60.4} & \underline{36.7} & \underline{73.7} & 11.7 & \textbf{37.1} & \textbf{7.8} & \textbf{2.7} & \textbf{47.7} & \textbf{34.6} & \textbf{20.9} & \textbf{46.0} & \textbf{7.9}  & 113.6 & 83.8 & 72.0 & 19.4 & 4.7 & \underline{119.0} & 56.7 & \underline{51.2} & 84.1 & 19.3 & 73.5 & 11.0 & 4.2 & 125.9 & 70.8 & 49.6 & 84.4 & 11.0 \\
        
        PROX~\cite{hassan2019resolving} & 86.1 & \underline{11.9} & \underline{5.6} & 189.1 & 86.2 & 83.5 & \underline{59.4} & \underline{10.5} & 4.6 & 161.1 & 66.4 & 53.9 & 75.8 & \underline{10.7} & \underline{55.6} & 10.1 & \underline{4.2} & \underline{116.9} & 53.5 & 51.7 & \underline{65.5} & 10.3 & 104.3 & 72.8 & \underline{61.0} & 17.6 & \underline{3.4} & 140.2 & 57.3 & \underline{49.8} & \underline{66.2} & 17.4 & 64.0 & 10.3 & 4.3 & 108.3 & 60.1 & 45.3 & 68.6 & 10.3 \\
        
        CrowdPose~\cite{li2019crowdpose} & 94.0 & 21.7 & 19.8 & 189.7 & 85.3 & 91.4 & 86.9 & 21.8 & 21.4 & 132.2 & 73.1 & 50.9 & 137.4 & 19.9 & 83.3 & 18.7 & 19.7 & 139.8 & 64.3 & 54.6 & 104.9 & 16.8 & 113.7 & 80.6 & 88.1 & 25.1 & 20.8 & 162.7 & 68.2 & 67.0 & 112.5 & 23.9 & 76.4 & 21.3 & 19.2 & 141.2 & 65.5 & 63.1 & 85.0 & 19.5 \\
        
        EgoBody-MVSet~\cite{zhang2022egobody} & 79.6 & \underline{12.4} & \underline{5.0} & 176.5 & {81.7} & \underline{76.8} & 67.2 & 11.4 & \underline{4.3} & 191.4 & 68.0 & 52.9 & 93.2 & 11.6 & \underline{55.7} & \underline{9.5} & \underline{3.5} & \underline{113.3} & \underline{49.4} & \underline{44.9} & 69.3 & \underline{9.6} & \underline{96.6} & 67.6 & 72.8 & 19.4 & \underline{3.7} & 138.8 & 59.6 & \underline{49.8} & 87.1 & 19.3 & 57.7 & 11.2 & \underline{3.5} & 101.9 & 55.8 & \underline{42.5} & 66.1 & 11.2 \\
        
        MPI-INF-3DHP~\cite{mehta2017monocular} & 91.0 & \underline{11.9} & 6.2 & 199.1 & 89.9 & 93.8 & 79.0 & \underline{10.4} & 6.1 & 147.0 & 73.7 & 75.3 & 99.1 & \underline{10.5} & 66.8 & \underline{9.9} & 5.5 & 128.7 & 56.9 & 63.5 & 79.5 &\underline{10.1} & 105.8 & \underline{65.1} & 69.8 & 17.2 & \underline{3.9} & 152.7 & 61.6 & 69.4 & 83.1 & 16.9 & 59.1 & 10.4 & 4.8 & 127.8 & 60.1 & 68.3 & 60.7 & 10.3 \\
        
        UBody~\cite{lin2023one} & 96.1 & 14.2 & 5.8 & 194.4 & 87.1 & 99.4 & \textbf{31.9} & \textbf{9.6} & \textbf{2.7} & \textbf{43.7} & \textbf{39.3} & \textbf{19.1} & \textbf{37.7} & \textbf{9.8} & 64.0 & 11.9 & 4.4 & 123.2 & 52.5 & \underline{44.7} & 74.2 & 12.3 & 131.3 & 98.6 & 70.3 & 17.2 & 5.7 & 157.2 & 56.1 & 78.7 & 83.2 & 17.1 & 87.9 & \underline{9.2} & 4.6 & 145.1 & 63.3 & 79.6 & 103.3 & \underline{9.3} \\
        
        RICH~\cite{huang2022capturing} & 93.3 & \underline{12.1} & 6.0 & 182.7 & 83.7 & 79.3 & 77.4 & 11.2 & \underline{4.5} & 159.4 & 67.9 & 43.5 & 100.0 & 11.4 & 85.8 & \underline{9.7} & 4.9 & 138.9 & 56.0 & 47.6 & 109.4 & \underline{10.0} & 123.2 & 93.2 & 79.6 & 18.6 & 4.6 & 142.6 & 58.7 & \underline{45.3} & 104.7 & 18.5 & 74.3 & \underline{9.7} & 4.8 & 104.3 & 56.7 & \underline{43.3} & 87.4 & \underline{9.8} \\
        
        MuCo-3DHP~\cite{Mehta2018SingleShotM3} & 106.5 & 23.5 & 69.7 & 205.7 & 86.1 & 129.4 & 104.4 & 22.4 & 70.7 & 202.6 & 77.7 & 113.8 & 88.8 & 20.6 & 90.4 & 20.2 & 69.7 & 162.8 & 65.3 & 108.8 & \underline{67.8} & 18.4 & 104.4 & \underline{60.3} & 95.6 & 25.7 & 68.6 & 166.4 & 69.2 & 114.2 & 76.2 & 24.5 & 86.8 & 21.6 & 69.4 & 156.9 & 67.5 & 115.6 & \underline{56.1} & 19.8 \\
        
        InstaVariety~\cite{kanazawa2019learning} & 148.0 & 20.3 & 73.3 & 230.3 & 92.5 & 204.8 & 130.2 & 20.2 & 75.1 & 181.2 & 68.9 & 186.9 & \underline{66.9} & 19.0 & 133.3 & 17.8 & 74.1 & 172.6 & 68.2 & 182.9 & 74.3 & 16.6 & \underline{97.8} & \underline{62.5} & 139.5 & 24.8 & 73.1 & 189.1 & 69.1 & 186.9 & 81.7 & 24.0 & 134.7 & 20.5 & 73.5 & 165.7 & 74.1 & 184.4 & 70.1 & 19.3 \\
        
        BEHAVE~\cite{bhatnagar2022behave} & 86.1 & 15.2 & 13.7 & 182.8 & 84.2 & 86.3 & 83.5 & 15.5 & 12.8 & 212.7 & 80.4 & 54.7 & 115.2 & 16.0 & 133.3 & 17.8 & 74.1 & 172.6 & 68.2 & 182.9 & 74.3 & 16.6 & 116.1 & 71.2 & 91.2 & \textbf{14.4} & 14.0 & 167.1 & 56.8 & 60.8 & 115.8 & \textbf{14.3} & 66.6 & 11.7 & 13.1 & 127.1 & 63.9 & 54.4 & 71.5 & 12.1 \\
        
        UP3D~\cite{lassner2017unite} & 95.3 & 21.7 & 18.1 & 228.3 & 97.8 & 97.8 & 80.0 & 20.5 & 19.0 & 181.4 & 89.6 & 58.0 & 97.8 & 18.5 & 82.6 & 18.3 & 17.8 & 160.3 & 74.9 & 59.2 & 95.2 & 16.4 & 142.4 & 96.6 & 91.2 & 24.4 & 18.1 & 197.3 & 77.7 & 80.2 & 113.6 & 23.0 & 84.6 & 20.5 & 18.1 & 173.5 & 79.7 & 73.0 & 98.4 & 18.7 \\
        
        ARCTIC~\cite{fan2023arctic} & 117.8 & 15.0 & 6.9 & 250.8 & 108.9 & 123.7 & 73.7 & 13.3 & 6.4 & 152.3 & 78.3 & 52.3 & 79.2 & 13.4 & 78.5 & 11.5 & 6.1 & 135.8 & 60.1 & 49.2 & 88.6 & 11.5 & 174.6 & 102.4 & \textbf{44.6} & 19.1 & \underline{3.4} & \textbf{71.2} & \textbf{42.5} & \textbf{37.2} & \textbf{47.1} & 19.1 & 87.1 & 13.2 & 5.8 & 172.7 & 87.5 & 93.7 & 88.9 & 13.0 \\
        
        3DPW~\cite{von2018recovering} & 88.9 & 33.7 & 17.6 & 190.8 & 89.3 & 91.9 & 82.9 & 35.2 & 14.6 & 218.2 & 88.2 & 56.2 & 106.9 & 32.1 & 75.1 & 35.9 & 15.1 & 143.6 & 73.6 & 60.0 & 82.9 & 32.9 & \underline{95.4} & 67.4 & 96.7 & 31.8 & 17.0 & 154.7 & 65.3 & 71.1 & 120.5 & 29.6 & 67.6 & 33.3 & 17.8 & 107.3 & 73.9 & 60.4 & 60.9 & 30.2 \\
        
        OCHuman~\cite{zhang2019pose2seg} & 109.0 & 25.2 & 18.4 & 216.1 & 95.6 & 110.4 & 89.3 & 22.7 & 18.5 & 199.3 & 83.4 & 63.7 & 122.1 & 20.8 & 98.4 & 20.4 & 16.8 & 165.9 & 71.9 & 64.6 & 115.9 & 18.7 & 157.0 & 112.3 & 101.6 & 25.0 & 17.7 & 191.3 & 68.2 & 71.7 & 124.5 & 23.8 & 105.2 & 23.7 & 17.3 & 172.8 & 83.0 & 85.5 & 114.2 & 21.6 \\
        
        CHI3D~\cite{fieraru2020three} & 75.4 & 18.6 & \underline{5.7} & 192.2 & 78.2 & 87.1 & 82.7 & 19.8 & 5.2 & 267.6 & 99.5 & 58.9 & 89.6 & 20.6 & 77.2 & 21.8 & 5.1 & 180.3 & 78.1 & 60.7 & 85.4 & 22.9 & 103.7 & \underline{64.9} & 81.5 & \underline{15.6} & 4.4 & 168.0 & 69.5 & 53.9 & 86.5 & \underline{15.7} & \underline{52.3} & 16.5 & \underline{4.0} & \underline{98.9} & 54.0 & 45.2 & \underline{53.0} & 17.1 \\
        
        DNA-R.-HiRes~\cite{renbody} & 90.1 & 14.7 & 6.1 & 210.2 & 80.5 & 111.4 & 79.5 & 12.9 & 5.0 & 267.3 & 66.1 & 77.9 & 106.1 & 13.3 & 76.4 & 12.4 & 4.6 & 181.9 & 57.0 & 67.3 & 96.2 & 12.8 & 125.4 & 77.3 & 72.6 & 17.5 & 5.0 & 161.9 & \underline{53.5} & 52.9 & 84.9 & 17.5 & \textbf{33.1} & \textbf{5.6} & \textbf{2.6} & \textbf{41.7} & \textbf{28.8} & \textbf{21.6} & \textbf{39.2} & \textbf{5.7} \\
        
        MTP~\cite{muller2021self} & 107.3 & 12.5 & 7.3 & 229.7 & 104.6 & 113.7 & 89.7 & 11.2 & 7.1 & 206.3 & 83.0 & 50.8 & 116.9 & 11.2 & 99.5 & \underline{10.0} & 6.7 & 169.4 & 65.9 & 56.3 & 135.2 & 10.1 & 181.0 & 116.8 & 109.9 & 17.8 & 6.3 & 184.7 & 66.3 & 76.8 & 151.5 & 17.6 & 100.5 & 10.9 & 6.2 & 177.3 & 87.4 & 95.9 & 120.3 & 10.8 \\
        
        HumanSC3D~\cite{fieraru2021learning} & 94.4 & 18.4 & 6.4 & 201.3 & 84.8 & 90.6 & 95.7 & 19.1 & 6.5 & 310.2 & 74.9 & 91.1 & 145.0 & 19.7 & 84.7 & 21.2 & 5.6 & 180.5 & 66.8 & 66.1 & 113.2 & 22.1 & \underline{99.2} & 70.6 & 94.5 & \underline{15.9} & 6.3 & 177.4 & 61.5 & 56.2 & 118.9 & \underline{16.0}& 60.8 & 16.9 & 4.8 & 114.5 & 60.1 & 52.8 & 60.8 & 17.4 \\
        
        DNA-Rendering~\cite{renbody} & 90.9 & 14.3 & 6.8 & 204.1 & 78.9 & 92.9 & 86.9 & 12.5 & 6.0 & 267.3 & 82.3 & 66.3 & 107.7 & 12.8 & 89.1 & 12.2 & 5.9 & 219.7 & 66.2 & 70.7 & 108.4 & 12.6 & 131.0 & 92.8 & 85.6 & 17.5 & 7.1 & 177.7 & 57.5 & 54.9 & 98.7 & 17.4 & 58.1 & \underline{6.6} & 5.1 & \underline{77.4} & \underline{38.7} & \underline{33.4} & 72.1 & \underline{6.7} \\
        
        FIT3D~\cite{fieraru2021aifit} & 114.4 & 19.3 & 5.9 & 253.3 & 93.1 & 106.5 & 100.9 & 19.5 & 5.8 & 299.3 & 88.1 & 62.0 & 129.3 & 20.1 & 90.6 & 21.6 & 5.3 & 201.7 & 68.4 & 64.6 & 110.0 & 22.4 & 111.9 & 75.9 & 95.4 & 15.9 & 5.5 & 237.6 & 65.6 & 83.5 & 108.0 & \underline{15.9} & 72.2 & 17.4 & 4.4 & 140.1 & 64.1 & 63.0 & 75.2 & 17.7 \\
        
        MPII~\cite{andriluka14cvpr}  & 155.5 & 33.6 & 16.3 & 252.5 & 107.6 & 131.0 & 120.5 & 34.9 & 16.2 & 227.8 & 91.5 & 90.7 & 161.6 & 31.7 & 129.1 & 35.7 & 16.3 & 211.8 & 90.9 & 96.8 & 148.9 & 32.6 & 183.3 & 147.0 & 129.1 & 31.6 & 15.8 & 232.0 & 83.4 & 138.8 & 149.3 & 29.4 & 142.7 & 33.2 & 15.6 & 205.6 & 102.5 & 121.8 & 157.7 & 30.0 \\
        
        Talkshow~\cite{yi2023generating} & 109.6 & 13.7 & 6.8 & 281.3 & 128.4 & 132.0 & 72.3 & 12.3 & 4.6 & \underline{125.6} & 66.6 & \underline{42.1} & 106.0 & 12.2 & 94.2 & 11.1 & 5.3 & 188.4 & 76.9 & 53.2 & 115.2 & 11.2 & 283.1 & 140.9 & 128.7 & 18.8 & 6.6 & 271.5 & 82.2 & 89.1 & 164.4 & 18.4 & 105.7 & 13.6 & 5.0 & 255.3 & 116.8 & 115.7 & 125.6 & 13.3 \\
        
        Human3.6M~\cite{ionescu2013human3} & 108.5 & 33.6 & 20.1 & 236.2 & 104.6 & 112.1 & 98.9 & 35.0 & 21.1 & 321.7 & 99.4 & 99.9 & 138.2 & 31.8 & 98.4 & 35.8 & 21.4 & 215.3 & 101.6 & 85.1 & 120.8 & 32.7 & 116.7 & 74.2 & 98.6 & 31.6 & 20.5 & 229.3 & 91.7 & 74.3 & 113.1 & 29.4 & 78.2 & 33.1 & 20.2 & 136.5 & 99.5 & 73.0 & 69.9 & 30.0 \\
        
        SSP3D~\cite{Sengupta2020SyntheticTF} & 165.2 & 33.9 & 19.4 & 261.8 & 111.4 & 187.3 & 151.0 & 35.4 & 18.2 & 244.0 & 125.4 & 197.6 & 180.1 & 32.1 & 165.4 & 36.2 & 18.2 & 238.5 & 108.9 & 211.8 & 181.1 & 32.9 & 242.9 & 167.8 & 165.7 & 31.6 & 17.8 & 297.1 & 101.8 & 236.9 & 182.8 & 29.2 & 165.5 & 33.3 & 18.6 & 245.3 & 108.7 & 187.9 & 173.1 & 30.0 \\
        
        LSPET~\cite{Johnson2011LearningEH} & 207.0 & 36.9 & 23.1 & 345.2 & 107.0 & 207.6 & 188.2 & 38.4 & 23.3 & 322.5 & 116.9 & 145.4 & 257.1 & 33.6 & 209.0 & 40.3 & 23.2 & 322.4 & 103.8 & 148.3 & 273.9 & 35.7 & 353.6 & 271.1 & 238.0 & 32.2 & 23.7 & 372.5 & 96.9 & 176.9 & 330.4 & 28.4 & 223.1 & 35.6 & 22.9 & 343.9 & 108.3 & 197.8 & 303.5 & 30.5 \\
        
      \bottomrule
    \end{tabular}}
\end{sidewaystable}


==> tables/inf_speed.tex <==
\begin{wraptable}{r}{0.3\textwidth}
  \vspace{-0.2cm}
  \caption{\textbf{Inference speed}. We tested the inference speed of the SMPLer-X model family on a single V100 GPU and presented the inference speed in FPS (frames per second).}
  \label{tab:inf_speed}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{lc}
    \toprule

    Method & FPS \\
    \midrule
    
    OSX~\cite{lin2023one} & 12.2 \\
    
    \name-S &  36.2 \\
    
    \name-B & 33.1 \\
    
    \name-L & 24.4 \\

    \name-H & 17.5 \\
    
    \bottomrule
  \end{tabular}}
\end{wraptable}


